Provably Bounding Neural Network Preimages

Most work on the formal verification of neural networks has focused on bounding the set of outputs that correspond to a given set of inputs (for example, bounded perturbations of a nominal input). However, many use cases of neural network verification require solving the inverse problem, or over-approximating the set of inputs that lead to certain outputs. We present the INVPROP algorithm for verifying properties over the preimage of a linearly constrained output set, which can be combined with branch-and-bound to increase precision. Contrary to other approaches, our efficient algorithm is GPU-accelerated and does not require a linear programming solver. We demonstrate our algorithm for identifying safe control regions for a dynamical system via backward reachability analysis, verifying adversarial robustness, and detecting out-of-distribution inputs to a neural network. Our results show that in certain settings, we find over-approximations over 2500x tighter than prior work while being 2.5x faster. By strengthening robustness verification with output constraints, we consistently verify more properties than the previous state-of-the-art on multiple benchmarks, including a large model with 167k neurons in VNN-COMP 2023. Our algorithm has been incorporated into the $\alpha,\!\beta$-CROWN verifier, available at https://abcrown.org.

==> feedback-queue.tex <==
- Give breathing room to OOD benchmark in results
- accurate discussion of branching

? - Remove R


==> sections/derivation-parallelogram.tex <==
We now prove the generalized theorem. As a conceptual overview of our proof, we take the Lagrange dual of the linear program to derive an unconstrained optimization problem. From here, we derive constraints that must be satisfied in the $\max \min$ formulation. These constraints yield the bound propagation procedure we display in Theorem \ref{thm:gamma-crown}.

We start with the LP of the convex relaxation. $$\begin{aligned}
\min _{\bsx, \hat{\bsx}, \mathbf{z}} \quad &  \bs{c}^{(0)\top}\hat{\bsx}^{(0)} + \sum_{i=1}^{L-1}\bs{c}^{(i)\top}\bsx^{(i)} \\
\text { s.t. } \quad &  \bs{l}^{(0)} \leq \hat{\bsx}^{(0)} \leq \bs{u}^{(0)} \\
& \bsx^{(L)} \leq \boldsymbol{0} ; \\
& \bsx^{(i)} =\mathbf{W}^{(i)} \hat{\bsx}^{(i-1)}+\mathbf{b}^{(i)} ; \quad i \in[L], \\
& \hat{x}_j^{(i)} \geq 0 ; j \in \mathcal{I}^{\pm(i)} \\
& \hat{x}_j^{(i)} \geq x_j^{(i)} ; j \in \mathcal{I}^{\pm(i)} \\
& \hat{x}_j^{(i)} \leq u_j^{(i)} z_j^{(i)} ; j \in \mathcal{I}^{\pm(i)} \\
& \hat{x}_j^{(i)} \leq x_j^{(i)}-l_j^{(i)}\left(1-z_j^{(i)}\right) ; j \in \mathcal{I}^{\pm(i)} \\
& \hat{x}_j^{(i)} =x_j^{(i)} ; j \in \mathcal{I}^{+(i)} \\
& \hat{x}_j^{(i)} =0 ; j \in \mathcal{I}^{-(i)} \\
& 0 \leq z_j^{(i)} \leq 1 ; \quad j \in \mathcal{I}^{\pm(i)}, i \in[L]
\end{aligned}$$

From this, we take the Lagrange dual of most of the constraints. In doing so, we introduce a new dual variable for each constraint. Note that we do not dualize every constraint since they can easily be dealt with later.

$$\begin{aligned}
\min_{\bsx, \hat{\bsx}, \mathbf{z}} \max_{\boldsymbol{\nu}, \boldsymbol{\mu}, \boldsymbol{\tau}, \boldsymbol{\gamma}, \boldsymbol{\pi}, \boldsymbol{\lambda}} \quad & \bs{c}^{(0)\top}\hat{\bsx}^{(0)} + \sum_{i=1}^{L-1}\bs{c}^{(i)\top}\bsx^{(i)} + \boldsymbol{\gamma}^{\top}\bsx^{(L)}+\sum_{i=1}^L \boldsymbol{\nu}^{(i) \top}\left(\bsx^{(i)}-\mathbf{W}^{(i)} \hat{\bsx}^{(i-1)}-\mathbf{b}^{(i)}\right) \\
& +\sum_{i=1}^{L-1} \sum_{j \in \mathcal{I}^{\pm(i)}}\left[\mu_j^{(i)}\left(-\hat{x}_j^{(i)}\right)+\tau_j^{(i)}\left(x_j^{(i)}-\hat{x}_j^{(i)}\right)\right. \\ & +\left.\lambda_j^{(i)}\left(\hat{x}_j^{(i)}-u_j^{(i)} z_j^{(i)}\right)+\pi_j^{(i)}\left(\hat{x}_j^{(i)}-x_j^{(i)}+l_j^{(i)}-l_j^{(i)} z_j^{(i)}\right)\right] \\
\text { s.t. }  \bs{l}^{(0)} & \leq \hat{\bsx}^{(0)} \leq \bs{u}^{(0)} ; \quad \hat{x}_j^{(i)} = 0, j \in \mathcal{I}^{-(i)} ; \quad \hat{x}_j^{(i)}=x_j^{(i)}, j \in \mathcal{I}^{+(i)} ; \quad 0 \leq z_j^{(i)} \leq 1, j \in \mathcal{I}^{\pm(i)} \\
\boldsymbol{\mu} & \geq 0 ; \quad \boldsymbol{\tau} \geq 0 ; \quad \boldsymbol{\gamma} \geq 0 ; \quad \boldsymbol{\pi} \geq 0 ; \quad \boldsymbol{\lambda} \geq 0
\end{aligned}$$

Since we took the dual of a linear program, the solution to the min-max optimization is equivalent to the solution of the max-min optimization by strong duality. Therefore, we can solve the following program (equivalent up to rearrangement).

$$\begin{aligned}
\max_{\boldsymbol{\nu}, \boldsymbol{\mu}, \boldsymbol{\tau}, \boldsymbol{\gamma}, \boldsymbol{\pi}, \boldsymbol{\lambda}} \min_{\bsx, \hat{\bsx}, \mathbf{z}} \quad &  \left(\boldsymbol{\nu}^{(L)}+\boldsymbol{\gamma}\right)^T \bsx^{(L)} + \left(\bs{c}^{(0)\top} - \boldsymbol{\nu}^{(1) \top} \mathbf{W}^{(1)}\right)\hat{\bsx}^{(0)} \\
& +\sum_{i=1}^{L-1} \sum_{j \in \mathcal{I}^{+(i)}}\left(\nu_j^{(i)}-\boldsymbol{\nu}^{(i+1) \top} \mathbf{W}_{:, j}^{(i+1)} + c^{(i)}_j\right) x_j^{(i)} +\sum_{i=1}^{L-1} \sum_{j \in \mathcal{I}^{-(i)}}\left(\nu_j^{(i)} + c^{(i)}_j\right) x_j^{(i)} \\
& +\sum_{i=1}^{L-1} \sum_{j \in \mathcal{I}^{\pm(i)}}\left[\left(\nu_j^{(i)}+\tau_j^{(i)}-\pi_j^{(i)}+c_j^{(i)}\right) x_j^{(i)}\right. \\
& +\left(-\boldsymbol{\nu}^{(i+1) \top} \mathbf{W}_{:, j}^{(i+1)}-\mu_j^{(i)}-\tau_j^{(i)}+\lambda_j^{(i)}+\pi_j^{(i)}\right) \hat{x}_j^{(i)} \\
& \left.+\left(-u_j^{(i)} \lambda_j^{(i)}-l_j^{(i)} \pi_j^{(i)}\right) z_j^{(i)}\right] \\
& -\sum_{i=1}^L \boldsymbol{\nu}^{(i) \top} \mathbf{b}^{(i)}+\sum_{i=1}^{L-1} \sum_{j \in \mathcal{I}^{\pm(i)}} \pi_j^{(i)} l_j^{(i)} \\
\text { s.t. }  \bs{l}^{(0)} & \leq \hat{\bsx}^{(0)} \leq \bs{u}^{(0)} ; \quad 0 \leq z_j^{(i)} \leq 1, j \in \mathcal{I}^{\pm(i)} \\
\boldsymbol{\mu} & \geq 0 ; \quad \boldsymbol{\tau} \geq 0 ; \quad \boldsymbol{\gamma} \geq 0 ; \quad \boldsymbol{\pi} \geq 0 ; \quad \boldsymbol{\lambda} \geq 0
\end{aligned}$$

We seek to remove the remaining constraints. We note that for $z^{(i)}_j$ constrained to $[0, 1]$, if the coefficient is positive, we should set $z^{(i)}_j = 0$. Otherwise, we should set $z^{(i)}_j = 1$ (if the coefficient is non-positive).

We also note that to minimize  $\left(\bs{c}^{(0)\top}-\boldsymbol{\nu}^{(1) \top} \mathbf{W}^{(1)}\right)\hat{\bsx}^{(0)}$ subject to $\bs{l}^{(0)} \leq \hat{\bsx}^{(0)} \leq \bs{u}^{(0)}$, we can consider the choice we must make in each dimension. If the $j$th entry of the coefficient is positive, we should set $\hat{x}^{(0)}_j = l^{(0)}_j$. Otherwise, we should set $\hat{x}^{(0)}_j = u^{(0)}_j$.

We reflect these observations in the following program by replacing their terms by equivalent representations.

$$\begin{aligned}
\max_{\boldsymbol{\nu}, \boldsymbol{\mu}, \boldsymbol{\tau}, \boldsymbol{\gamma}, \boldsymbol{\pi}, \boldsymbol{\lambda}} \min_{\bsx, \hat{\bsx}} \quad &  \left(\boldsymbol{\nu}^{(L)}+\boldsymbol{\gamma}\right)^T \bsx^{(L)}+\ReLU\left(\bs{c}^{(0)\top} - \boldsymbol{\nu}^{(1) \top} \mathbf{W}^{(1)}\right)\bs{l}^{(0)}-\ReLU\left(-\bs{c}^{(0)\top} +\boldsymbol{\nu}^{(1) \top} \mathbf{W}^{(1)}\right)\bs{u}^{(0)} \\
& +\sum_{i=1}^{L-1} \sum_{j \in \mathcal{I}^{+(i)}}\left(\nu_j^{(i)}-\boldsymbol{\nu}^{(i+1) \top} \mathbf{W}_{:, j}^{(i+1)} + c^{(i)}_j\right) x_j^{(i)} +\sum_{i=1}^{L-1} \sum_{j \in \mathcal{I}^{-(i)}}\left(\nu_j^{(i)} + c^{(i)}_j\right) x_j^{(i)} \\
& +\sum_{i=1}^{L-1} \sum_{j \in \mathcal{I}^{\pm(i)}}\left[\left(\nu_j^{(i)}+\tau_j^{(i)}-\pi_j^{(i)} + c^{(i)}_j\right) x_j^{(i)}\right. \\
& +\left(-\boldsymbol{\nu}^{(i+1) \top} \mathbf{W}_{:, j}^{(i+1)}-\mu_j^{(i)}-\tau_j^{(i)}+\lambda_j^{(i)}+\pi_j^{(i)}\right) \hat{x}_j^{(i)} \\
& \left.- \ReLU\left(u_j^{(i)} \lambda_j^{(i)}+l_j^{(i)} \pi_j^{(i)}\right)\right] \\
& -\sum_{i=1}^L \boldsymbol{\nu}^{(i) \top} \mathbf{b}^{(i)}+\sum_{i=1}^{L-1} \sum_{j \in \mathcal{I}^{\pm(i)}} \pi_j^{(i)} l_j^{(i)} \\
\text { s.t. } \boldsymbol{\mu} & \geq 0 ; \quad \boldsymbol{\tau} \geq 0 ; \quad \boldsymbol{\gamma} \geq 0 ; \quad \boldsymbol{\pi} \geq 0 ; \quad \boldsymbol{\lambda} \geq 0
\end{aligned}$$

From here, we note that the variables $\bs{x}$ or $\hat{\bs{x}}$ are unconstrained variables. Therefore, if any of their coefficients are nonzero, the inner minimization can immediately drive its value to $-\infty$. As such, the outer maximization must set all of these coefficients to zero. Therefore, we can derive constraints from this restructured optimization and remove the free variables $\bs{x}, \hat{\bs{x}}$.

$$\begin{aligned}
\max_{\boldsymbol{\nu}, \boldsymbol{\mu}, \boldsymbol{\tau}, \boldsymbol{\gamma}, \boldsymbol{\pi}, \boldsymbol{\lambda}} \quad & \ReLU\left(\bs{c}^{(0)\top} - \boldsymbol{\nu}^{(1) \top} \mathbf{W}^{(1)}\right)\bs{l}^{(0)}-\ReLU\left(-\bs{c}^{(0)\top} +\boldsymbol{\nu}^{(1) \top} \mathbf{W}^{(1)}\right)\bs{u}^{(0)} -\sum_{i=1}^L \boldsymbol{\nu}^{(i) \top} \mathbf{b}^{(i)}\\
&+ \sum_{i=1}^{L-1} \sum_{j \in \mathcal{I}^{\pm(i)}}\left[\pi_j^{(i)} l_j^{(i)} - \ReLU\left(u_j^{(i)} \lambda_j^{(i)}+l_j^{(i)} \pi_j^{(i)}\right) \right] \\
\text { s.t. } \quad 
\boldsymbol{\nu}^{(L)} &= -\boldsymbol{\gamma} \\
\nu_j^{(i)} &= \boldsymbol{\nu}^{(i+1) \top} \mathbf{W}_{:, j}^{(i+1)} - c^{(i)}_j, j \in \mathcal{I}^{+(i)} \\
\nu_j^{(i)} &= - c^{(i)}_j, j \in \mathcal{I}^{-(i)} \\
\nu_j^{(i)} &= \pi_j^{(i)} - \tau_j^{(i)} + c^{(i)}_j, j \in \mathcal{I}^{\pm(i)} \\
\boldsymbol{\nu}^{(i+1) \top} \mathbf{W}_{:, j}^{(i+1)} &= \left(\lambda_j^{(i)}+\pi_j^{(i)}\right)-\left(\mu_j^{(i)}+\tau_j^{(i)}\right), j \in \mathcal{I}^{\pm(i)} \\
\boldsymbol{\mu} & \geq 0 ; \quad \boldsymbol{\tau} \geq 0 ; \quad \boldsymbol{\gamma} \geq 0 ; \quad \boldsymbol{\pi} \geq 0 ; \quad \boldsymbol{\lambda} \geq 0
\end{aligned}$$

For the following, we define $\hat{\nu}^{(i)}_j = \boldsymbol{\nu}^{(i+1) \top} \mathbf{W}_{:, j}^{(i+1)}$. We note that since the upper and lower bounds of the neuron relaxation can not be tight simulataneously, at least one of $\lambda^{(i)}_j + \pi^{(i)}_j$ and $\mu^{(i)}_j + \tau^{(i)}_j$ must be non-zero \footnote{Similar to the observation in \citealt{zhang2022general, wong2018provable}, both may be non-zero in theory if our $l^{(i)}_j$ and $u^{(i)}_j$ are perfectly tight. However, this is rarely the case and loosening our bounds by an arbitrarily small constant suffices.}. Therefore, we can write them as $\lambda^{(i)}_j + \pi^{(i)}_j = [\hat{\nu}^{(i)}_j]_+ $ and $ \mu^{(i)}_j + \tau^{(i)}_j = [\hat{\nu}^{(i)}_j]_-$

If we choose $\pi^{(i)}_j = \frac{u}{u-l}[\hat{\nu}^{(i)}_j]_+$ and $\lambda^{(i)}_j = \frac{-l}{u-l}[\hat{\nu}^{(i)}_j]_+$ and observe that $\tau^{(i)}_j$ lies in the interval $0$ and $\hat{\nu}^{(i)}_j$, we get the following bound propagation procedure.

$$\begin{aligned}
\max_{\boldsymbol{\nu}, \bs{\alpha}, \boldsymbol{\gamma}} \quad & \ReLU\left(\bs{c}^{(0)\top} - \boldsymbol{\nu}^{(1) \top} \mathbf{W}^{(1)}\right)\bs{l}^{(0)}-\ReLU\left(-\bs{c}^{(0)\top} +\boldsymbol{\nu}^{(1) \top} \mathbf{W}^{(1)}\right)\bs{u}^{(0)} -\sum_{i=1}^L \boldsymbol{\nu}^{(i) \top} \mathbf{b}^{(i)}\\
& + \sum_{i=1}^{L-1} \sum_{j \in \mathcal{I}^{\pm(i)}}\left[\frac{u^{(i)}_{j}l^{(i)}_j [\hat{\nu}^{(i)}_j]_{+}}{u^{(j)}_{i} - l^{(j)}_i} \right] \\
\text { s.t. } \quad
\boldsymbol{\nu}^{(L)} &= -\boldsymbol{\gamma} \\
\nu_j^{(i)} &= \boldsymbol{\nu}^{(i+1) \top} \mathbf{W}_{:, j}^{(i+1)} - c^{(i)}_j, j \in \mathcal{I}^{+(i)} \\
\nu_j^{(i)} &= - c^{(i)}_j, j \in \mathcal{I}^{-(i)} \\
\hat{\nu}_j^{(i)} &= \boldsymbol{\nu}^{(i+1) \top} \mathbf{W}_{:, j}^{(i+1)} \\
\nu_j^{(i)} &= \frac{u^{(i)}_{j}}{u^{(j)}_{i} - l^{(j)}_i}[\hat{\nu}^{(i)}_j]_{+} - \alpha^{(i)}_j[\hat{\nu}^{(i)}_{j}]_{-} + c^{(i)}_j, j \in \mathcal{I}^{\pm(i)} \\
\alpha^{(i)}_j & \in [0, 1] ; \quad \boldsymbol{\gamma} \geq 0
\end{aligned}$$

In this program, $\alpha^{(i)}_j$ are optimizable parameters controlling the relaxation of neuron $j$ in layer $i$, similar to the ones appearing in \citealt{xu2021fast}. $\bs{\gamma}$, as discussed in the body of the paper, is the parameter which enforces the output constraint throughout this entire bound propagation procedure. 
